Progressive Weight Pruning of Deep Neural Networks using ADMM

Deep neural networks (DNNs) although achieving human-level performance in many domains, have very large model size that hinders their broader applications on edge computing devices. Extensive research work have been conducted on DNN model compression or pruning. However, most of the previous work took heuristic approaches. This work proposes a progressive weight pruning approach based on ADMM (Alternating Direction Method of Multipliers), a powerful technique to deal with non-convex optimization problems with potentially combinatorial constraints. Motivated by dynamic programming, the proposed method reaches extremely high pruning rate by using partial prunings with moderate pruning rates. Therefore, it resolves the accuracy degradation and long convergence time problems when pursuing extremely high pruning ratios. It achieves up to 34 times pruning rate for ImageNet dataset and 167 times pruning rate for MNIST dataset, significantly higher than those reached by the literature work. Under the same number of epochs, the proposed method also achieves faster convergence and higher compression rates. The codes and pruned DNN models are released in the link bit.ly/2zxdlss

==> 2_background.tex <==
\section{Background}



\subsection{Related Work on Weight Pruning}

\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-0.2in}
\begin{center}
	\includegraphics[width = 0.4\textwidth]{Fig_pruning.pdf}
    %\vspace{-0.35in}
	\caption{Illustration of DNN weight pruning.}
	\label{fig:pruning}
\end{center}
\vspace{-0.25in}
\end{wrapfigure}

\textbf{Weight pruning} methods leverage the inherent redundancy in the number of weights in DNNs, thereby achieving effective model compression with negligible accuracy loss, as illustrated in Fig. \ref{fig:pruning}. 
A pioneering work of weight pruning is \cite{han2015learning}. 
It uses a heuristic, iterative method to prune the weights with small magnitudes and retrain the DNN. 
It achieves 9$\times$ weight reduction on AlexNet for ImageNet dataset, without accuracy degradation. 
However, this work achieves relatively low compression ratio (2.7$\times$ for AlexNet) on the CONV layers, which are the key computational part in state-of-the-art DNNs \cite{simonyan2015very,he2016deep}. 
Besides, indices are needed, at least one per weight, to index the relative location of the next weight. 
To address these limitations, this work has been extended in two directions.
The first is improving the weight reduction ratio by using more sophisticated heuristics, e.g., incorporating both weight pruning and growing \cite{guo2016dynamic}, using $L_1$ regularization method \cite{wen2016learning}, or genetic algorithm \cite{dai2017nest}. 
The second is enhancing the actual implementation efficiency. 
This goal is achieved by either deriving an effective tradeoff between accuracy and compression ratio, e.g., the \emph{energy-aware pruning} \cite{yang2017designing}, or incorporating regularity and structures into the weight pruning framework, e.g., the \emph{channel pruning} \cite{he2017channel} and \emph{structured sparsity learning} \cite{wen2016learning} approaches.



% \textbf{Pros and cons of the two methods:} Weight quantization has clear advantage: it is hardware-friendly. 
% The computation requirement is reduced in proportion to weight representation, and multiplication operations can be eliminated using binary/ternary quantizations. 
% On the other hand, weight pruning incurs inevitable implementation overhead due to the irregular sparsity and indexing \cite{han2015deep,wen2016learning,yu2017scalpel,yang2017designing,ding2017c}.  

The major advantage of weight pruning is the higher potential gain in model compression. 
The reasons are two folds. 
First, there is often higher degree of redundancy in the number of weights than bit representation. 
In fact, reducing each bit in weight presentation doubles the imprecision, which is not the case in pruning. 
Second, weight pruning performs regularization that strengthens the salient weights and prunes the unimportant ones. 
It can even increase the accuracy with a moderate pruning ratio \cite{wen2016learning,han2016dsd}. 
As a result it provides a higher margin of weight reduction. 
%This effect does not exist in weight quantization/clustering. 

% \textbf{Combination:} Because they leverage different sources of redundancy, weight pruning and quantization can be effectively combined. 
% However, there lacks a systematic investigation in this direction. 
% The extended work \cite{han2015deep} by Han \emph{et al.} uses a combination of weight pruning and clustering (not quantization) techniques, achieving 27$\times$ model compression on AlexNet. 
% This compression ratio has been updated by the recent work \cite{zhou2017incremental} to 53$\times$ on AlexNet (but without any specification about compressed model).


% \subsection{Other Work on DNN Model Compression}

% There are also some other methods for DNN model compression.
% The low-rank matrix approximation method \cite{sainath2013low} assumes low-rank weight matrices and uses factorization to present a low-rank weight matrix by two smaller matrices, and thereby reducing the number of parameters. 
% \cite{chung2016simplifying} integrates the matrix factorization with weight pruning.
% And the low-rank matrix approximation has also been investigated with focus on speed up test-time evaluation \cite{denton2014exploiting}.
% Similar approach or namely singular vector decomposition has been extended to acoustic models and memristor-based neuromorphic computing \cite{xue2013restructuring,liu2015eda}.

% Another branch of work on DNN model compression is representing weights using structured matrices \cite{sindhwani2015structured}, in particular by using circulant weight matrices \cite{cheng2015exploration}, and block-circulant weight matrices \cite{}.



 
\subsection{Basics of ADMM}

ADMM has been demonstrated \cite{ouyang2013stochastic,suzuki2013dual} as a powerful tool for solving non-convex optimization problems, potentially with combinatorial constraints.
Consider a non-convex optimization problem that is difficult to solve directly. 
ADMM method decomposes it into two subproblems that can be solved separately and efficiently. 
For example, the optimization problem
\begin{equation}\label{eqn:1}
   \min_{\bf{x}}\ \ f({\bf{x}})+g({\bf{x}})
\end{equation}
lends itself to the application of ADMM if $f(\bf{x})$ is differentiable and $g(\bf{x})$ has some structure that can be exploited. 
Examples of $g(\bf{x})$ include the $L_1$-norm or the indicator function of a constraint set. 
The problem is first re-written as
\begin{equation}
\label{eqn:2}
\begin{aligned}
& \min_{\bf{x},\bf{z}}
& & f(\textbf{x})+g(\textbf{z}),
\\ & \text{subject to}
& & \bf{x}=\bf{z}.
\end{aligned}
\end{equation}
Next, by using augmented Lagrangian \cite{boyd2011distributed}, the above problem is decomposed into two subproblems on $\bf{x}$ and $\bf{z}$. 
The first is $\min_{\bf{x}} f({\bf{x}})+q_1(\bf{x})$, where $q_1(\bf{x})$ is a quadratic function. 
As $q_1(\bf{x})$ is convex, the complexity of solving subproblem 1 (e.g., via stochastic gradient descent) is the same as minimizing $f(\bf{x})$. 
Subproblem 2 is $\min_{\bf{z}} g({\bf{z}})+q_2(\bf{z})$, where $q_2(\bf{z})$ is a quadratic function. 
When function $g$ has some special structure, exploiting the properties of $g$ allows this problem to be solved analytically and optimally. 
In this way we can get rid of the combinatorial constraints and solve the problem that is difficult to solve directly.




